Evaluation of probabilistic photometric redshift estimation approaches for The Rubin Observatory Legacy Survey of Space and Time (LSST)

Many scientific investigations of photometric galaxy surveys require redshift estimates, whose uncertainty properties are best encapsulated by photometric redshift (photo-z) posterior probability density functions (PDFs). A plethora of photo-z PDF estimation methodologies abound, producing discrepant results with no consensus on a preferred approach. We present the results of a comprehensive experiment comparing twelve photo-z algorithms applied to mock data produced for The Rubin Observatory Legacy Survey of Space and Time (LSST) Dark Energy Science Collaboration (DESC). By supplying perfect prior information, in the form of the complete template library and a representative training set as inputs to each code, we demonstrate the impact of the assumptions underlying each technique on the output photo-z PDFs. In the absence of a notion of true, unbiased photo-z PDFs, we evaluate and interpret multiple metrics of the ensemble properties of the derived photo-z PDFs as well as traditional reductions to photo-z point estimates. We report systematic biases and overall over/under-breadth of the photo-z PDFs of many popular codes, which may indicate avenues for improvement in the algorithms or implementations. Furthermore, we raise attention to the limitations of established metrics for assessing photo-z PDF accuracy; though we identify the conditional density estimate (CDE) loss as a promising metric of photo-z PDF performance in the case where true redshifts are available but true photo-z PDFs are not, we emphasize the need for science-specific performancemetrics.

==> authors.tex <==
% Author list file generated with: mkauthlist 1.2.3 
% mkauthlist -j mnras -f -c LSST Dark Energy Science Collaboration --cntrb contributions.tex authors.csv authors.tex 

\author[LSST Dark Energy Science Collaboration]{
\parbox{\textwidth}{
\Large
S.J.~Schmidt$^{1}$\thanks{Email: sschmidt@physics.ucdavis.edu},
A.I.~Malz$^{2,3,4}$\thanks{Email: aimalz@astro.ruhr-uni-bochum.de},
J.Y.H.~Soo$^{5,6}$,
I.A.~Almosallam$^{7,8}$,
M.~Brescia$^{9}$,
S.~Cavuoti$^{9,10}$,
J.~Cohen-Tanugi$^{11}$,
A.J.~Connolly$^{12}$,
J.~DeRose$^{13,14,15,16,17}$,
P.E.~Freeman$^{18}$,
M.L.~Graham$^{12}$,
K.G.~Iyer$^{19,20}$,
M.J.~Jarvis$^{21,22}$,
J.B.~Kalmbach$^{12}$,
E.~Kovacs$^{23}$,
A.B.~Lee$^{18}$,
G.~Longo$^{10}$,
C.B.~Morrison$^{12}$,
J.A.~Newman$^{24}$,
E.~Nourbakhsh$^{1}$,
E.~Nuss$^{11}$,
T.~Pospisil$^{18}$,
H.~Tranin$^{11}$,
R.H.~Wechsler$^{25,16,26}$,
R.~Zhou$^{15,24}$,
R.~Izbicki$^{27,28}$
\begin{center} (LSST Dark Energy Science Collaboration) \end{center}
}
\vspace{0.4cm}
\\
\parbox{\textwidth}{
(Affiliations are listed at the end of the paper)
\vspace{0.8cm}
}
}

